Exploiting co-execution with oneAPI: heterogeneity from a modern perspective

Programming efficiently heterogeneous systems is a major challenge, due to the complexity of their architectures. Intel oneAPI, a new and powerful standards-based unified programming model, built on top of SYCL, addresses these issues. In this paper, oneAPI is provided with co-execution strategies to run the same kernel between different devices, enabling the exploitation of static and dynamic policies. On top of that, static and dynamic load-balancing algorithms are integrated and analyzed. This work evaluates the performance and energy efficiency for a well-known set of regular and irregular HPC benchmarks, using an integrated GPU and CPU. Experimental results show that co-execution is worthwhile when using dynamic algorithms, improving efficiency even more when using unified shared memory.

==> background.tex <==

% JL: Nota general de Jose Luis, refiriéndose a toda la sección de "model"
% Esto hay que dejarlo en una página más o menos. Es el background, no es nada nuestro y por lo tanto el que quiera saber más que vaya a las referencias. Está bien escrito y puede servir para otra ocasión o incluso tu tesis, pero para el artículo es muy largo. Tenemos que centrarnos en lo que vamos a usar en el resto del artículo.

% untouched: means does not differ from the "model" version

%\subsection{OneAPI Execution Model}

% TODO: mostly untouched, unless first sentence  and the single source prop removed. Maybe reduce?
OneAPI is based on the SYCL specification, although it provides its own extensions to accelerate the computation and facilitate the development. Its programming language is called Data Parallel C++ (DPC++), making a leap in abstraction and promoting interoperability with host code.
%JLB: , compared to the OpenCL language. DPC++ is a community-driven, standards-based language built on ISO C++ and Khronos SYCL, allowing developers to reuse code across hardware targets.
% DPC++ allows the host and the device code as part of the same compilation unit, feature called single
%source property, that allows potential optimizations across the boundary between both codes. Due to this property,
DPC++ establish three types of scope to distinguish between host (application), host-device interface (command group) and device (kernel). OneAPI comprises four models based on SYCL.
%JLB: , each of which is part of the operations that a developer has to take when using oneAPI.

\subsubsection{Platform model}

% removed examples of API and code references
Define a host that manages one or more devices and coordinates the application and command group scopes. A device can be an accelerator or the CPU itself, each of which contains a set of Compute Units, each of these provides one or more processing elements. The complete system could have multiple platforms, since the composition of drivers in execution platforms is determined by the drivers and its implementation.

\subsubsection{Execution model}

It defines and specifies how kernels execute on the devices and interact with the host. It is subdivided in host and device execution models. The data management and execution between host and devices are coordinated by the host execution model via command groups. These are groupings of commands like kernel invocation and accessors, which are submitted to queues for execution. 
%JLB: Queues are declared and instantiated, which issue command groups under in-order (SYCL 2020) or out-of-order policies (default mechanism).
% TODO: maybe reduce more?
%JLB: No he visto que se use en el resto del artículo. Se puede compactar más o incluso eliminar, si hace falta espacio.
The device execution model specifies how computation is accomplished on the accelerator, specifying range data sets. These are allocated across a hierarchy of ND-ranges, work-groups, sub-groups, and work-items, easing the programming patterns and their composition.
%of operations for each program. 
%JLB: This facilitates the memory and compute operation relationships, giving the programmer flexibility to express the algorithms.

%JLB: Mirar si se puede compactar las dos últimas frases, parece que dicen cosas similares. 
% Technically: DPC++ runtime 
A fundamental concept in the SYCL execution model is the Directed Acyclic Graph (DAG). Each node contains an action to be performed on a device, such as kernel invocation or data movements. The SYCL runtime controls resolution of dependencies and triggering of node executions, asynchronously. Thus, it tracks and orchestrates actions and their dependencies to perform in the devices, safely executing each operation when the requirements are met.

%Each command group submitted to a queue contain a single handler, which is the responsible to track the programmer's
%requested actions and establish relationships and dependencies between operations. 
%
%JLB: On the other side, if the handler is not used, the code executes synchronously by the CPU as part of the host program, bypassing the DAG.

% PAPER: Probablemente nos carguemos el DAG y el listing/código, dejándolo para la revista
% PAPER: eliminados los subgroups

\subsubsection{Memory model}

It coordinates the allocation and management of memory between the host and devices, and how they interact. Memory resides upon and is owned by either the host or the device and is specified by declaring a memory object. {\em Accessors} define the interaction of these memory objects between host and device, communicating the desired location and access mode.

An extension to the standard SYCL memory model is Unified Shared Memory (USM), which enables the sharing of memory between the host and devices without explicit accessors. It manages access and enforces dependencies with explicit functions to wait on events or by signaling a dependency relationship between events. Another important feature of USM is that it provides a C++ pointer-based alternative to the buffer programming model, which increases the abstraction by leaving the migration of memory to the underlying runtime and device drivers. On the other side, since it does not rely on accessors, dependencies between command group operations must be specified using events to help the compiler determine the data dependencies and patterns.

\subsubsection{Kernel programming model}

The kernel is the computing function instantiated to be executed by every processing element of the accelerator. It allows the
programmer to determine what code executes on the host and device, giving an explicit computing function via lambda expression, functor or kernel class. Therefore, the separation of host and device codes is straightforward, without language extensions. Device code can specify the parallelism mechanism with a coarse-grained task, data-parallel work or data-parallel work taking into consideration the hierarchical range of the execution model. 
It supports the single source property, meaning the host code and device code can be in the same source file. 
%JLB It improves usability, safety between host and device boundaries (matching kernel arguments) and optimization strategies due to better understanding of the execution context (aliasing inference, propagating constants).

% TODO: remove?

%JLB: Se puede eliminar todo. 
Finally, DPC++ kernels execute asynchronously via forced allocations of kernel class instances, implicit waits of C++ destructors or explicit queue waits. 

% TODO: he eliminado el Compilation Model entero

